ViStruct: Simulating Expert-Like Reasoning Through Task Decomposition and Visual Attention Cues

Data visualization tasks often require multi-step reasoning, and the interpretive strategies experts use, such as decomposing complex goals into smaller subtasks and selectively attending to key chart regions are rarely made explicit. ViStruct is an automated pipeline that simulates these expert behaviours by breaking high-level visual questions into structured analytic steps and highlighting semantically relevant chart areas. Leveraging large language and vision-language models, ViStruct identifies chart components, maps subtasks to spatial regions, and presents visual attention cues to externalize expert-like reasoning flows. While not designed for direct novice instruction, ViStruct provides a replicable model of expert interpretation that can inform the development of future visual literacy tools. We evaluate the system on 45 tasks across 12 chart types and validate its outputs with trained visualization users, confirming its ability to produce interpretable and expert-aligned reasoning sequences.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January and March 2023

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unix-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/chartTaskSelection.tex <==
\subsection{Chart and Task Selection}



chart selection: 

% We focus exclusively on static visualizations rather than interactive or animated charts to maintain a controlled environment that ensures consistency across participants and allows for reliable gaze pattern analysis. Interactive visualizations introduce variability in user behavior, making it difficult to determine whether gaze paths are driven by cognitive processing of the visualization or interaction-based decisions. Additionally, different data relationships induce distinct gaze behaviors, as spatial visualizations (e.g., choropleth maps) direct attention differently than magnitude-based visualizations (e.g., bar charts). Selecting charts with different dimensionalities (univariate, bivariate, multivariate) enables a comparative analysis of gaze structures across simple and complex data encodings, while incorporating multiple representation styles (charts, graphs, maps, networks) ensures comprehensive coverage of how visual form influences systematic gaze paths.

% We build on VLAT's validated set of 12 chart types, which categorizes low-level analytic tasks across diverse visualization types, including charts (bar, line, pie, area), graphs (scatterplots, bubble charts), maps (choropleth), and hierarchical structures (treemaps). However, to eliminate redundancy, we remove Scatterplots (redundant with Bubble Charts), Area Charts (redundant with Line and Stacked Area Charts), and Stacked Bar Charts (redundant with Standard and 100\% Stacked Bar Charts), as they do not introduce distinct gaze behaviors. To enhance diversity, we add Sankey Diagrams (flow-based path tracking), Parallel Coordinates Plots (multivariate structured scanning), and Violin Plots (density-distribution comparisons), ensuring a broader spectrum of gaze patterns across visualization types, encodings, and cognitive demands.

we focus exclusively on static visualizations rather than interactive or animated charts. While interactive charts are common in modern data visualization, static charts provide a controlled environment that ensures consistency across participants and allows for more reliable gaze pattern analysis. Including interactive visualizations would introduce variability in user behavior, making it difficult to determine whether gaze paths are driven by the underlying cognitive processing of the visualization or the interactions themselves.

Different data relationships create unique areas of interest (AOIs) and induce varied eye movement patterns. For example, spatial visualizations like choropleth maps differ significantly from magnitude visualizations such as bar charts in how they direct user attention. 
https://arxiv.org/html/2502.03575v1

The Financial Times Visual Vocabulary provides a rigorous foundation for selecting diverse charts as it employs distinct visual structures, ensuring that we evaluate gaze behavior across all major data interpretation contexts.

selecting charts with different dimensionalities (univariate, bivariate, multivariate) allows us to compare simple vs complex gaze structure.

we also need to make sure gaze behavior is tested across multiple representation styles (charts, graphs, maps, networks)

VLAT provides a well-structured and validated set of 12 chart types, making it an ideal foundation for studying systematic gaze paths in data interpretation. One of the primary advantages of using VLAT is that it already categorizes different visualization tasks and assigns them to specific visualization types, ensuring that a broad spectrum of cognitive operations is represented.

VLAT charts span multiple visualization types, including:

Charts (bar charts, line charts, pie charts, area charts)
Graphs (scatterplots, bubble charts)
Maps (choropleth maps)
Hierarchical visualizations (treemaps)

VLAT also accounts for different dimensionalities:

Univariate (histogram, bar chart, pie chart)
Bivariate (line chart, scatterplot, choropleth map)
Multivariate (bubble chart, stacked bar chart, treemap)


Moreover, the visual encodings used in VLAT charts are diverse, covering:
Points (scatterplots, bubble charts)
Lines (line charts, area charts)
Bars (bar charts, stacked bar charts, histograms)
Areas (choropleth maps, treemaps)

While the VLAT charts provide a strong foundation, some visualizations introduce redundancy without offering additional interpretative challenges or distinct gaze behaviors. To ensure that each selected chart provides a unique contribution to gaze pattern analysis, we propose removing Scatterplot, Area Chart, and Stacked Bar Chart due to their similarity with existing charts:

Scatterplot (Remove)

Redundant with Bubble Chart: Both require users to compare points along x-y axes, but Bubble Charts add size encoding, increasing cognitive complexity.
No Additional Gaze Challenge: Since both charts involve free search patterns, keeping only Bubble Charts maintains the same analysis benefits while reducing redundancy.
Area Chart (Remove)

Redundant with Line Chart and Stacked Area Chart: Area Charts encode trends over time, just like Line Charts, but do not introduce a unique gaze path.
Stacked Area Chart Adds Complexity: Stacked Area Charts require users to track multiple layers, whereas Area Charts only emphasize a single series, making them less useful.
Stacked Bar Chart (Remove)

Too Similar to Standard Bar Chart: Users still compare bar heights in the same way, making the gaze structure almost identical to a standard Bar Chart.
100\% Stacked Bar Chart Is More Informative: Since 100\% Stacked Bar Charts force relative proportion comparisons, they offer more distinct gaze path variations than standard Stacked Bar Charts.

To ensure a diverse set of gaze behaviors, we introduce visualizations that add new cognitive demands, require different scanpaths, and improve representation across visualization types. These new charts will enhance interpretation challenges and fill gaps left by the removed charts:

Sankey Diagram (Add)

Introduces Flow-Based Gaze Behavior: Unlike any VLAT chart, Sankey diagrams require path-following gaze movements between linked entities.
Tracks Hierarchical Relationships: Instead of static comparisons, users must trace how data flows between categories, adding a new type of gaze interaction.
Parallel Coordinates Plot (Add)

Expands Multivariate Analysis: While Bubble Charts add size encoding, Parallel Coordinates Plots visualize multiple variables across vertical axes, forcing users to shift gaze between intersecting lines.
Encourages Comparative Eye Movements: Unlike scatterplots, which allow free searching, parallel coordinates force structured scanning across multiple attributes.
Violin Plot (Add)

Alternative for Distribution Analysis: Histograms (kept in VLAT) only show count distributions, but Violin Plots combine density estimation with category comparison, introducing different gaze movements.
Balances Local \& Global Comparisons: Users must switch between the center of each distribution (for density patterns) and edges (for range estimation), creating a more layered gaze path structure.




task selection: 
Retrieve Value
• Filter
• Compute Derived Value
• Find Extremum
• Sort
• Determine Range
• Characterize Distribution
• Find Anomalies
• Cluster
• Correlate

Since VLAT already categorizes visualization tasks into low-level analytical components, we adopt its framework to ensure standardized, validated task selection. These tasks are designed to assess fundamental cognitive operations when interpreting visual data, covering a range of difficulty levels and cognitive demands. 

\subsection{Procedure}




\subsection{Participant}

demographic, familiarities, number of participants, compensation paid

==> sections/conclusion.tex <==
In conclusion, we present \textbf{ViStruct}, an automated pipeline that simplifies visualization tasks by decomposing them into semantically meaningful subtasks, extracting structured region information, and providing step-by-step visual guidance. The prototyped system is deployed and can be accessed \href{https://vi-struct.vercel.app/}{here}. Our evaluation shows reliable performance across diverse static charts and tasks. We plan to enhance flexibility with context-aware guidance and extend the approach to interactive settings to better support insight extraction.



==> sections/designGoals.tex <==
In the initial stage of designing ViStruct, our goal was to deeply understand expert strategies in visualization problem-solving, which are essential to support expert-like behavior effectively. To achieve this, we considered both how experts approach visualization tasks and the specific challenges novices face when attempting similar tasks. Prior research highlights that experts typically approach charts by systematically attending to semantically meaningful regions and interpreting them in a structured sequence \cite{moerth_kostic_gehlenborg_pfister_beyer_nobre_2025}. In contrast, novices often face difficulties accurately interpreting visual encodings, misreading visual channels, confusing chart labels with data values, and struggling to formulate data-driven visual queries \cite{Rezaie2024, Lee2016, Grammel2010, nobre_24}. Understanding these differences helped us identify the key aspects of expert reasoning that ViStruct should support. The design goals for ViStruct are:\\
\textbf{G1: Semantic Region Understanding} During the encoding stage of visualization comprehension, experts naturally identify and interpret distinct semantic regions of a chart (axes, data marks, and labels) to extract relevant visual information \cite{brunye_eye_2020}. Effective encoding requires accurately understanding each region's roles within the visual structure \cite{nobre_24}. Therefore, the system needs to detect these components accurately and assign labels that meaningfully reflect each component's function. \\
\textbf{G2: Precise Coordinate Mapping} In the decoding stage, the visual elements identified must be translated into their corresponding quantitative meanings. This process involves precisely mapping spatial features, such as the height of bars or the positions of data points, to numerical values through alignment with reference regions and axis scales \cite{nobre_24}. The system must support this decoding step so that users can interpret the quantitative information embedded within the spatial arrangement of chart components.\\
\textbf{G3: Structured Task Decomposition} 
Complex visualization tasks are combinations of low-level analytic components that require integration to reveal underlying insights\cite{amar_low-level_nodate}. There are many ways to combine these elements, and the system should provide a step-by-step decomposition that aligns with expert reasoning. This structured guidance helps novices manage complex visual analysis by reducing information overload. \cite{Grammel2010, Kerren2020}.\\
\textbf{G4: Supporting Diverse Data Encoding}
Charts use a wide range of symbols, layouts, and dimensional mappings to encode data; each may call for a different approach to interpretation\cite{boner2019}. To support diverse chart types and visualization tasks, the system must accurately classify chart components by integrating information from both textual descriptions and geometric shapes.\\
\textbf{G5: Interpretability and Transparency}
Every stage of the reasoning process should be clearly explained to improve interpretability. This includes how regions are divided, what data is extracted, and why certain decisions are made. ViStruct enhances this process using visual attention guidance \cite{jamet_attention_2008, xie_more_2017}, such as highlights and circled AOIs, to direct users toward task-relevant areas. These visual cues allow users to follow the model's interpretation path.



==> sections/discussion.tex <==
\textbf{Varying Effectiveness of Guidance Across Task Types:} Our evaluation showed that the AOI-based guidance works well for concrete tasks such as filtering or locating values, where visual cues are direct. However, AOIs alone are less effective for more abstract tasks (i.e., correlation). These tasks require integrating multiple elements, suggesting that richer cues, such as tooltips or side panels, may be more appropriate. Future work should explore customized guidance strategies through participatory design or user feedback.


\\\textbf{Supporting Diverse Reasoning Paths and Scaffolding:} While the ViStruct decomposition strategy is effective for many tasks, it may not always match how users reason about complex visualizations. Abstract tasks often permit multiple valid approaches, so a fixed breakdown can be limiting. Future work should enable flexible, user‑driven reasoning by adding an interactive chatbot that refines task flows, clarifies goals, and adapts strategies to each chart. It should also provide scaffolded explanations that explain why each step matters, instead of always splitting tasks into their smallest parts, so novices can build a deeper conceptual understanding.


\\\textbf{Guiding Novices and Reducing Cognitive Load:} ViStruct’s structured task decomposition and visual guidance aim to simulate expert-like reasoning, helping novices manage cognitive load and navigate complex charts. Our study evaluated whether this technique could reproduce expert insights in realistic usage scenarios. Future work should assess its impact on learning outcomes, usability, and task performance, especially for novice users in educational settings.
% \\\textbf{Limitations in Static Chart Processing:} ViStruct is currently designed for static, raster-based charts, relying on OpenCV to detect regions from a single image. This approach limits its effectiveness in interactive environments, where visualizations frequently change in response to user actions. Future work should focus on supporting task decomposition for insight extractions across multiple coordinated views, as commonly seen in platforms like Tableau or Vega-Lite dashboards. 



% \textbf{Scalability and Reasoning Efficiency for Extremum Tasks} 
% \\The system currently needs to receive all values in the chart to determine maximum or minimum values. This brute-force method works for charts such as bar or pie charts because they always have limited categories. However, this approach becomes inefficient for large, dense visualizations like scatter plots. Expert analysts take a different approach. They scan the value axis strategically, from top to bottom, to find the maximum and then map it back to the corresponding visual element. This efficient, expert-like heuristic type is not yet captured in the model's reasoning process. Future work should explore ways to improve reasoning efficiency, including tuning or fine-tuning the LLM to simulate more strategic search behaviour and better scale to complex visualizations.

% Also mention the flexibility in other tasks like retrieve values as well, for example, some would prefer to use the minus bar to extract, and some use the combinations. 
% mention the ability with a realtime chat bot for explaaning the different options.
% \\\textbf{Varying Effectiveness of Guidance Across Task Types} 
% \\Building on the above challenge, our evaluation revealed that specific low-level component tasks, such as filtering and value retrieval, are well-suited to AOI-based guidance. Users can easily follow the visual cues to complete these steps with minimal ambiguity. In contrast, more abstract tasks such as computing derived values (e.g., proportions or differences) were less intuitive with AOI alone. We propose that strategies like hover-over tooltips, summary panels showing derived results, or overlays such as trendlines may better support tasks requiring comparison or aggregation. Future work should involve participatory design sessions or user workshops to explore and refine tailored guidance strategies for each subtask type.




==> sections/evaluation.tex <==
We conducted two evaluations to assess ViStruct’s effectiveness as an expert-like visual reasoning pipeline: a performance evaluation to test decomposition accuracy and scalability and an expert evaluation to understand user perceptions regarding clarity, usefulness, and expert-like behaviour.

\vspace{-2mm}
\subsection{Performance Evaluation} 
\vspace{-1mm}
We tested ViStruct on 45 visualization tasks drawn from \hyperlink{https://bckwon.pythonanywhere.com/}{VLAT} and \hyperlink{https://tools.visualdata.wustl.edu/experiment/\#/}{Mini-VLAT}, covering all 12 chart types (\textbf{G4}). Each task was executed five times, resulting in 225 trials. For each trial, we evaluated ViStruct’s ability to identify semantic chart regions (\textbf{G1}), map visual features to data values (\textbf{G2}), and generate coherent task decompositions (\textbf{G3}). ViStruct produced correct outputs in 192 of the 225 trials (85.33\%). It performed consistently on concrete tasks such as value lookup and filtering. In contrast, more abstract tasks such as correlation analysis in multidimensional charts (i.e., bubble charts) occasionally showed inconsistencies by selecting the wrong visual channels for analysis.

\vspace{-2mm}
\subsection{Expert Review}
\vspace{-1mm}
 We conducted an expert evaluation to assess whether ViStruct demonstrates expert-like behaviour and provides valuable guidance. Each participant was assigned three charts and could select any task from the question bank. They evaluated ViStruct's decomposition, workflow logic, region identification, and visual guidance. Specifically, they rated ViStruct on: \textit{(1)} usefulness for novice users, \textit{(2)} accuracy of subtasks and AOIs, and \textit{(3)} alignment with their reasoning. Participants also gave open-ended feedback and used a think-aloud protocol during tasks.

 We recruited 20 participants (12 males, 8 females), including 12 undergraduates in a data visualization course, 4 graduate researchers, and 4 industry data analysts. All participants were screened for familiarity with surveyed chart types and reported an average rating of 6.35 out of 7. Each session lasted 30 minutes, and participants received a \$10 gift card.

 
\textbf{Experts' Perceptions and Feedback.}
Participants rated ViStruct highly for guiding visual reasoning (\textit{M = 6.14, SD = 1.38}); the accuracy of its decompositions and AOIs scored 5.93 (\textit{SD = 1.58}), and its perceived expert‑likeness was 5.97 (\textit{SD = 1.53}).

\textbf{Step-by-step guidance supported participants in organizing their reasoning.} Several users noted that the combination of visual overlays and sequential explanations clarified how to approach complex charts. One participant remarked that “\textit{visual overlays alongside explanatory text is a useful step‑by‑step guide... especially with bubble charts where there are more variables than people are used to}” (\textit{p14}). This form of guided interaction helped participants build a mental model of the task structure (\textbf{G2, G5}).

\textbf{Region annotations anchored users' attention to relevant chart elements.} Participants appreciated the system’s ability to highlight and label specific visual components (\textbf{G1}). Numbered regions were especially helpful for less experienced users, who found the annotations reduced confusion (\textbf{G5}). One participant commented that “\textit{the mapping feature... helps visually guide them in each step by highlighting the regions to focus on}” (\textit{p9}).

\textbf{Experts interpreted the decomposition as instructional guidance aimed at novice users.} While many agreed that the step-by-step breakdown resembled how they would teach a novice (\textbf{G3}), they did not feel the need to follow every step themselves. One participant observed that “\textit{the steps were clear and resemble how a domain expert would interpret and guide someone}” (\textit{p3}). In contrast, some others noted that “\textit{for experienced people, some of the steps might be a bit too detailed, but someone who is new to these charts could find it very helpful}” (\textit{p8}).

\textbf{Participants suggested refining phrasing and allowing control over guidance depth.} Suggestions included making instructions sound more natural, such as replacing “Filter a month on the x-axis” with “focus on each month” (\textit{p6}), and introducing grouping or modular breakdowns to reduce cognitive load in complex tasks (\textit{p2}).






==> sections/intro.tex <==
Decomposing a complex task into smaller, manageable components is widely recognized as an effective strategy for problem-solving \cite{briakou2024, fischer2012process, Kazemitabaar2024Improving, stepbystep, Morrison2015Subgoals}. Experts often perform such decomposition intuitively, but novices typically struggle without explicit guidance\cite{Nelms2019ExpertNovice}. Consequently, interfaces that provide structured support through clear task organization and intermediate goals have been shown to improve problem-solving efficiency and promote deeper reasoning across different domains \cite{Tullis2015Scheduling, Kazemitabaar2025Improving}. 

Data visualization tasks also involve complex reasoning and involve multiple cognitive stages \cite{Lee2016}. However, these steps are rarely made explicit \cite{karer_2020}. High-level visualization goals are typically achieved through combinations of low-level component actions \cite{amar_low-level_nodate}. Studies show that experts can implicitly coordinate these subtasks using structured strategies \cite{teo_exploratory_2023, brunye_eye_2020}, whereas novices often struggle to identify or apply such patterns without explicit guidance. This gap underscores the need for structured task decomposition as a foundation for supporting users during visualization analysis. 

Expert-level guidance for visualization analysis remains challenging because task decomposition depends heavily on the specific visualization being used. Additionally, effective guidance must identify which Areas of Interest (AOIs) within the chart correspond to each subtask, requiring precise mapping between analytical steps and the visual regions containing the relevant information. Manually crafting these guidances is infeasible at scale due to the wide variability in visualization goals, subtasks, and chart designs. Although AI-driven approaches have successfully decomposed complex tasks in other domains \cite{tankelevitch2024metacognitive, suh2023sensecape}, their potential for decomposing visualization-specific tasks and delivering precise visual attention guidance remains largely unexplored.

To bridge this gap, we introduce \textbf{ViStruct}, an automated AI-driven technique specifically designed to generate expert-like, step-by-step guidance for visualization tasks. ViStruct leverages large-language (LLM) and vision-language models (VLM) to systematically \textbf{decompose visualization tasks}, dynamically \textbf{identify context-specific AOIs}, and effectively \textbf{produce actionable instructional sequences} tailored to the structure and semantics of the chart.

To validate the scalability of the proposed technique, we applied it to 45 visualization tasks across 12 chart types. We evaluated our approach with 20 domain experts, confirming the expert-like guidance and transparency provided by ViStruct. The resulting technique is publicly available as an open-source interactive platform for researchers and practitioners, accessible \href{https://vi-struct.vercel.app/}{here}.

==> sections/relatedWork.tex <==
% \subsection{AI’s Role in User Engagement for Learning}

% from passive observer to active learners

% user engagement in learning systems

% ai for scaffoloding and feedback

% challenges in ai driven engagement for info vis


% main structure:

% shows existing works shows how Ai guided user engagement in structured learning

% AI-driven adaptive learning systems have been widely explored for fostering user engagement in education and interactive systems.
% However, research on AI’s role in engaging users in exploratory, data-driven environments such as information visualization is limited.
% Unlike structured learning tasks, InfoVis engagement involves self-directed exploration, making it unclear whether AI should proactively guide users or allow for autonomy. Understanding AI’s impact on engagement in InfoVis is essential for designing adaptive visualization systems.

% \subsection{The Debate Between Reactive and Proactive Assistive Systems}

% AI-driven assistive systems can either wait for user requests (reactive) or intervene before the user struggles (proactive)



% \subsection{LLMs for Information Visualization as guiding tool}

% LLM enhance data literact on demand, it can be serve as a guide for novices in chart interpretation

% Q and A systems, chart understanding
Our work draws upon related efforts in AI-driven reasoning frameworks for task decomposition and in vision-language approaches for spatial and semantic understanding of data visualizations. 
\subsection{AI Assisted Task Decomposition}
Previous research has investigated how AI can assist in task decomposition. For example, Chain-of-Thought \cite{wei2022chain} prompting aids in reasoning traces, and ReAct \cite{yao2023react} combines reasoning with external actions. These techniques are integrated into Talk2Data \cite{guo2024talk2data} and LightVA \cite{zhao2024lightva} as an interactive system for visual analysis and task planning. Some approaches also emphasize user control and trust by allowing users to guide and verify the decomposition process through interactive steps \cite{Kazemitabaar2024Improving}, highlighting the importance of transparency and interpretability in AI-assisted reasoning. 

Similarly, in data visualization, frameworks also explored explainable AI decomposition \cite{yin2024data} and automated analytic workflow \cite{alves2024ai}. However, these tools often require users to request decomposition explicitly. Thus, they are more suited to experienced users who understand when and how to use these features effectively. In contrast, ViStruct offers automated, proactive task decomposition, helping novice users without needing expert-driven interaction. 

\subsection{Region-Aware Processing in Data Visualization}
Recent work reveals that while VLMs show some capability in interpreting chart structures and high-level relationships \cite{huang2024relationvlm}, they often lack consistency and robustness \cite{mukhopadhyay2024unraveling}. Many models struggle with understanding visual language and fail to capture relational information accurately, which is critical for interpreting charts \cite{hou2024vision}. Even advanced models still face challenges in reliably extracting meaningful visual relationships.

Newer approaches emphasize region-based understanding. MapReader\cite{zhang2025mapreader} demonstrates how spatial visualizations benefit from region-level segmentation, while intermediate text representations\cite{ye2024beyond} have been used to improve flowchart comprehension. With the help of \hyperlink{https://opencv.org/}{OpenCV}, the Chain-of-Region technique\cite{lichain} proposes explicitly segmenting charts into interpretable regions (axes, bars, legends, etc) and combining this with VLMs enables precise coordinate-to-region mapping, which is crucial for tasks like identifying the correct values in bar or line charts. 

ViStruct leverages region-based techniques by detecting semantically meaningful regions within charts and defining task-specific AOIs. Motivated by sequential visual cues (SVCs) \cite{sequantial}, which guide attention through critical regions in order, ViStruct integrates region segmentation directly into VLMs, aligning visual cues with each step of the task decomposition.

% \subsection{Visual Attention Guidance in Data Visualization} 
% Visual cues such as arrows, highlights, and coloured borders are widely used to direct people's attention to relevant information, improving focus, retention, and transfer of knowledge \cite{jamet_attention_2008, van_gog_signaling_2014, xie_more_2017}. 
% % Similarly, modelling expert gaze behaviour through instructional videos has been shown to enhance novice problem-solving accuracy across domains. \cite{jarodzka_learning_2013, gegenfurtner_effects_2017}.
% Several data visualization systems have attempted to support users by incorporating visual cues directly into visualizations. ChartAccent\cite{ChartAnnotation} supports adding annotations and automatically highlights salient data regions to draw attention to key insights. More recently, systems have begun detecting user confusion through facial expressions and offering real-time guidance in visual analytics\cite{showeye}. However, these rule-based approaches lack adaptability and expert-like strategies for complex tasks. ViStruct differs by generating task-specific AOIs in a structured sequence. This bridges the gap between static cues and dynamic, goal-driven guidance.





==> sections/system.tex <==
Considering the design requirements, we developed ViStruct as a prototype system to explore automated, expert-like reasoning of visualizations through chart decomposition and visual guidance. This section outlines the ViStruct pipeline and its integration, beginning with a user-facing scenario and then detailing each system component: chart characterization, task decomposition, region annotation, and attention-guided output. For each stage, we describe how it supports the design goals introduced in Section~\ref{goals}.

ViStruct is implemented as a prototype interactive platform using TypeScript and the Next.js framework, with a backend powered by OpenCV for region detection. The system is model-agnostic and adaptable to different vision-language models. In our initial experiments, we tested Gemini-2-Flash, GPT-4V, and Claude 3.7 on structured chart inputs at each stage of the pipeline. We selected Gemini-2-Flash for integration due to its faster response time and more reliable performance in understanding visual elements.


% \begin{figure}[htb]
%   \centering
%   \includegraphics[width=1\linewidth]{figs/overview.png}
%   \caption{\label{fig:overview}
%            Example workflow of ViStruct}
% \end{figure}

\subsection{Overview}
Given a static chart and a user-defined visualization task, ViStruct processes the input through a multi-stage pipeline. As shown in Figure~\ref{fig:teaser}, the system uses OpenCV and Gemini-2-Flash to detect the chart type, extract visual features, and identify geometric elements like bars, lines, axes, and text labels (Sec~\ref{sec:chart_characterization}). This information is passed to Gemini-2-Flash, which decomposes the task into smaller subtasks (Sec~\ref{sec:task_decomposition}). ViStruct then validates and organizes the subtasks, allowing optional user edits with semantic checks (Sec~\ref{sec:decomposition_flow}). The system labels chart regions based on this structure to enable pixel-to-semantics mapping (Sec~\ref{sec:region_identification}). These regions define task-specific AOIs to guide attention for each subtask (Sec~\ref{sec:visual_attention}). 

As the user progresses through the task at their own pace, they continuously select one subtask at a time, receive visual guidance via highlighted regions, complete the steps, and move on. 

\begin{figure}[htb]
  \centering
  \includegraphics[width=1\linewidth]{figs/decomposition.png}
  \caption{\label{fig:decomp}
           \textbf{(T) Task Decomposition:} The system presents a low-level component task breakdown derived from the user’s high-level question, categorized by task type. \textbf{(W) Editable Workflow Interface:} Users can view and manipulate the task structure and customize the workflow, selecting variable instances and reordering steps.}
\end{figure}

\vspace{-5mm}
\subsection{Usage Scenario} \label{sec:usage_scenario}
To illustrate how ViStruct supports expert-like visual reasoning, we present a usage scenario where a user analyzes an Olympic medal chart (Fig.~\ref{fig:decomp}). The chart is a 100\% stacked bar chart, where each bar represents a country's total medal count, subdivided into gold, silver, and bronze. The user wants to determine which country has the smallest proportion of gold medals.

After uploading the chart and asking, \textit{"Which country has the least proportion of gold medals?"}, ViStruct automatically detects the chart type and parses it into semantic regions such as bars, segments, axes, and legend. Each region is labelled with its meaning, supporting \textbf{G1} by enabling structured interpretation of visual elements. Users can click any segment to see a natural language description (e.g., \textit{Gold medal count for USA}), which reinforces semantic understanding.

ViStruct then decomposes the question into a sequence of low-level analytic tasks (Sec.~\ref{sec:task_decomposition}). For example, one subtask may involve identifying the top boundary of a country's gold segment to compute its proportion. The full task sequence is shown in Fig.~\ref{fig:decomp}. This structured breakdown supports \textbf{G3}, guiding users step-by-step through a complex visual query while reducing cognitive load.

To assist decoding, the system highlights segment boundaries and draws reference lines to help users map visual features to numeric values (Fig.~\ref{fig:teaser}e), supporting \textbf{G2}. Each subtask is interactive and editable; users can explore intermediate results, reorder steps, or focus on specific regions while maintaining logical coherence (Sec.~\ref{sec:decomposition_flow}). This transparency and control over the reasoning flow support \textbf{G5}, allowing users to follow and understand the system's decisions.

% To illustrate how ViStruct supports real-world visualization tasks, we present a usage scenario involving a user analyzing an Olympic medal distribution chart (Fig \ref{fig:teaser}). The user is given a 100\% stacked bar chart, where each bar represents a country and is divided proportionally into segments for gold, silver, and bronze medals. They aim to determine which country has the most minor proportion of gold medals relative to its total medal count.

% The user begins by uploading the chart and posing the question: \textit{"Which country has the least proportion of gold medals?"} ViStruct initiates the pipeline by first characterizing the chart type and layout (see Section~\ref{sec:chart_characterization}), identifying it as a stacked bar chart with normalized values. At the same time, the system begins parsing the chart into semantically meaningful regions, including axes, individual bar segments, and the legend, each labelled with its function. This supports \textbf{G1} and \textbf{G2}, where the system accurately detects and assigns functional labels to chart components to reflect their roles within the visual structure. Users can interactively explore these regions; selecting a segment will display its meaning in natural language (e.g., \textit{"This segment represents the gold medal count for USA"}).

% Next, the system decomposes the visualization task into low-level analytic subtasks (Section~\ref{sec:task_decomposition}), aligning with \textbf{G3}. For this specific question, the decomposition might include: \textit{Task 1 (Filter):} Identify the bar segment representing 'Gold' medals in the chart legend. \textit{Task 2 (Filter):} Identify a country on the x-axis. \textit{Task 3 (Retrieve Value):} Determine the bottom boundary of the 'Gold' segment for the country. \textit{Task 4 (Retrieve Value):} Determine the top boundary of the 'Gold' segment for the country. \textit{Task 5 (Compute Derived Value):} Subtract the bottom value from the top to compute the proportion of gold medals. \textit{Task 6 (Find Extremum):} Find the minimum value among all calculated proportions.

% An example workflow might complete \textit{Task 1}, then iterate \textit{Task 2} through \textit{5} for each country, and finally perform \textit{Task 6}. ViStruct presents this decomposition as an editable flow; the user may reorder or prioritize specific countries, and the system ensures the logic remains valid during any adjustments (see Section~\ref{sec:decomposition_flow}). This supports \textbf{G5}, allowing users to see and influence the system’s reasoning.

% After task decomposition and region labelling, the user can activate step-by-step guidance for any subtask. For example, in Task 4, the first visual cue may highlight the top boundary of the 'Gold' segment in a selected country's bar. Once acknowledged, the following guidance step may render a horizontal line extending from the segment to the y-axis, helping the user trace the value visually. These visual cues guide users' attention and explain how each task connects to the underlying data, contributing to both \textbf{G2} and \textbf{G5}. Users can move forward or backward through these guided steps, allowing replay or refinement of their thought process. This structured, interpretable flow supports both task completion and visual learning. Once the user finishes a given step, they can click "Finished" button to confirm completion and proceed to the next task in the sequence. This allows them to move through the entire decomposition at their own pace while maintaining continuity and context across the reasoning process.

\subsection{Chart Characterization} \label{sec:chart_characterization}
ViStruct begins by characterizing the input chart to extract its structural and semantic layout as a foundation for downstream reasoning. Gemini-2-Flash organizes them into a structured JSON representation, including axis ranges, variable names, data groupings, and encoding types.

To improve the reliability of OpenCV-based region detection, graphical elements are categorized into four shape types: line-based, dot-based, rectangular, and irregular. This classification allows ViStruct to adapt region analysis methods to the chart’s visual encoding scheme.

Chart characterization supports \textbf{G4} by enabling ViStruct to generalize across diverse chart types and visual conventions.

\subsection{Task Decomposition} \label{sec:task_decomposition}

ViStruct uses a multi-stage prompting framework with three sequential prompts to decompose high-level user tasks into low-level analytic subtasks. The LLM operates on a structured input that includes (1) the user's natural language query, (2) the JSON chart description (Sec.~\ref{sec:chart_characterization}), and (3) a list of labelled chart regions with spatial metadata.

Decomposition is guided by a predefined taxonomy of ten low-level task types\cite{amar_low-level_nodate}. The first prompt produces a breakdown based on this taxonomy. The second refines each step to ensure it is grounded in specific, executable, and sufficiently detailed chart regions. If a step is too abstract, the LLM splits it into atomic components. The third prompt validates the structure, resolves step dependencies, and removes redundant subtasks (e.g., repeating the same operation across different chart elements).

This breakdown–refine–verify process ensures each step is precise, executable, and aligned with the task structure. It directly supports \textbf{G3} by enabling structured task decomposition and \textbf{G4} by adapting reasoning to diverse chart types and visual encodings.

\subsection{Decomposition Flow Example} \label{sec:decomposition_flow}
Due to visual analysis's compositional nature, there is often no correct way to sequence low-level operations. ViStruct presents one example workflow based on the decomposition results (Fig.~\ref{fig:decomp}), illustrating a valid approach. Recognizing that users may prefer different reasoning paths, the system allows them to modify the sequence, adjust parameters, or reorganize tasks to fit their analysis strategy better. The LLM then validates the revised flow to ensure logical consistency. If valid, both the workflow and the underlying decomposed tasks are updated accordingly.

\begin{figure}[htb]
  \centering
  \includegraphics[width=1\linewidth]{figs/regionIdentification.png}
  \caption{\label{fig:region}
    \textbf{Workflow of region identification}: The input chart is processed using OpenCV to identify distinct regions corresponding to chart segments. These regions are labeled by the system. VLM then identifies each annotated region with meaningful descriptions.}
\end{figure}

\vspace{-6mm}
\subsection{Region Identification} \label{sec:region_identification}
Region identification is a key step in the ViStruct pipeline, providing the precise coordinate-level data needed for visual guidance and accurate annotation. To highlight AOIs during task execution, the system must first detect all meaningful chart components, including axes, labels, data marks, and legends.

The process begins with OpenCV-based text detection (Fig.~\ref{fig:region}), which identifies individual characters and outputs their bounding boxes (\texttt{x-min}, \texttt{x-max}, \texttt{y-min}, \texttt{y-max}). Characters with similar x- or y-values are grouped into complete text elements, allowing the system to reconstruct axis labels, ticks, and legend entries.

For non-text elements, OpenCV’s edge detection and colour segmentation identify visual regions such as bars, pie slices, or legend swatches based on shape boundaries and colour differences. In charts with continuous marks like lines or areas, the system uses identified axis ticks as reference points and interpolates pixel coordinates along the visual path to map data values.

This yields a complete set of region coordinates but without semantic meaning. To bridge this gap, the system overlays numbered labels on an annotated chart image and sends both the image and coordinate data to Gemini-2-Flash, which returns natural language descriptions for each region (e.g., \textit{"Gold medal for the USA"}). This transforms low-level visual segments into semantically meaningful components, directly supporting \textbf{G1} by identifying functional chart regions and \textbf{G2} by linking visual geometry to interpretable data values.

\vspace{-2mm}
\subsection{Visual Attention Guidance} \label{sec:visual_attention}
After chart regions are semantically identified, ViStruct generates step-by-step visual guidance to help users focus on relevant elements and understand how to extract the correct information from the chart.

To generate this guidance, the system provides the LLM with structured input: (1) the current low-level subtask, (2) a JSON object detailing chart regions, their coordinates, region IDS, and semantic labels, and (3) task-specific metadata from stage \ref {sec:chart_characterization}. Each of the subtask types uses an individual prompt to ensure contextual accuracy and clarity.

Based on this input, the LLM generates a sequence of visual guidance steps tied to specific regions or reference points. Some, like bar segments or axis labels, are directly retrieved from the JSON, while others involve simple geometric reasoning. For instance, the system draws a horizontal line from the bar’s edge to the y-axis to read a bar's top value, guiding the user’s attention.

ViStruct creates an interpretable and grounded guidance flow by combining textual instructions with precise visual markers. This directly supports \textbf{G2} by helping users connect spatial features to quantitative meaning and \textbf{G5} by making each reasoning step transparent and visually traceable.
